Interactive Movement Primitives: Planning to Push Occluding Pieces for Fruit Picking

Robotic technology is increasingly considered the major mean for fruit picking. However, picking fruits in a dense cluster imposes a challenging research question in terms of motion/path planning as conventional planning approaches may not find collision-free movements for the robot to reach-and-pick a ripe fruit within a dense cluster. In such cases, the robot needs to safely push unripe fruits to reach a ripe one. Nonetheless, existing approaches to planning pushing movements in cluttered environments either are computationally expensive or only deal with 2-D cases and are not suitable for fruit picking, where it needs to compute 3-D pushing movements in a short time. In this work, we present a path planning algorithm for pushing occluding fruits to reach-and-pick a ripe one. Our proposed approach, called Interactive Probabilistic Movement Primitives (I-ProMP), is not computationally expensive (its computation time is in the order of 100 milliseconds) and is readily used for 3-D problems. We demonstrate the efficiency of our approach with pushing unripe strawberries in a simulated polytunnel. Our experimental results confirm I-ProMP successfully pushes table top grown strawberries and reaches a ripe one.

==> intro.tex <==
\section{Introduction}
%\subsection*{Problem definition}
Among different motion planning strategies developed over the past years for robotic manipulation, 
few of them tackled the main problems still existing: reaching an object in cluttered and uncertain environment. The majority of state of art techniques will fail in generating feasible paths in such scenarios, e.g \cite{vahrenkamp2010integrated}. However, we can find recent works mostly devoted to manipulation in clutters. For example, in \cite{dogar2012planning}, a framework using non-prehensile actions, such as pushing actions, was proposed. The framework works under high uncertainty by utilizing the funneling effect of pushing. Similar approaches were proposed in \cite{kitaev2015physics}, \cite{king2015nonprehensile} and \cite{agboh2018real}. 


Similar environment can be also found in the agri-robotics sector, where robot harvesting still faces the challenge of picking fruits from clusters. The two main problems created by agriculture clusters are: occlusion facing the camera system and occlusion facing the robot end-effector.


In this work, we focus on the problem of picking fruits in clusters while dealing with the occlusion introduced to the end-effector path planning.

Labour shortage is a global increasing dilemma to the agriculture sector, e.g. United Kingdom (UK) agriculture industry is currently concerned about the future availability of labor for picking and the consequent inflation in labor cost due to Brexit. 
In UK, the soft fruit sector uses 29,000 seasonal pickers to generate over 160,000 tons of fruit every year \cite{xiong2019autonomous}. For example, only strawberry harvesting cost is more than $60\%$ of the total production cost \cite{Agri}. 
%e.g the total strawberry harvesting cost for the 2016 year at the central cost of California is $44,809\$$ per acre \cite{Agri}, constituting $66\%$ of the total cost $67,674\$$ \cite{Agri}. 
Adapting a robotic technology that is able to navigate to the field, monitor, detect and localize the ripe ones, and eventually pick and deliver them to a pack house, can be the remedy to every shortage. 

% While robotic automation is continuously growing in several areas, from logistics to domestic and aeronautics, giving hope for an increase in productivity and safety, a current shortage in agricultural labor has started to call for the need of mobile robots in outdoor fields to compensate for it 

%Aside labour shortage, autonomous robot harvesters can increase the production rate, thanks to the embedded intelligence that allows them to operate day and night and hence reduce human fatigue when harvest transportation is in question.

\begin{figure}[tb]\centering
\subfloat[]{\includegraphics[scale=0.025]{figs/s5.jpg}\label{fig:s1}}\hspace{0.01cm}
\subfloat[]{\includegraphics[scale=0.025, trim=0 0 0 0]{figs/s1.jpg}\label{fig:s2}}\hspace{0.01cm}
\subfloat[\label{fig:s3}]{\includegraphics[width = 3cm, height = 3.5cm, scale = 0.15]{dwg/picker.png}}
\caption{\ref{fig:s1} and \ref{fig:s2} show sample situations of the table top grown strawberries in which unripe strawberries occlude the approach from the bottom. The table top growing is getting popular because the growing condition can be precisely controlled. \ref{fig:s3} shows our strawberry picking robot consisting of a SCARA arm and a mobile robot, and harvesting in a simulated polytunnel ripe fruits from a cluster close to what we can face in condition \ref{fig:s1}. }\label{fig:graphs}
%\vspace*{-2mm}
\end{figure}


% \subsection*{Existing works}
An increasing trend in robotic harvesting is nowadays traced out. Schuetz et al. in \cite{schuetz2015evaluation} formulated the harvesting problem as a static optimal control problem relying on an initially generated heuristic trajectory. In their work, the authors generate an optimal harvesting trajectory that minimizes the collision and dynamical costs. In \cite{luo2018collision}, the authors presented an energy optimal combined with an artificial potential field approach to formalize the problem of a collision-free path-planning harvesting 6-DoFs robot.
In \cite{xiong2019autonomous}, the authors propose an active obstacle-separation path planning strategy for picking fruits in clusters inspired by human pickers who usually use their hands to push and separate surrounding obstacles during picking. 
%The latter strategy uses the pose of fruits within a region of interest (ROI) of a ripe fruit to define the obstacles. It divides the ROI into 12 subsections in the 3D space and then classifies the obstacle into bottom or top one. 
%In the latter work, the authors adapt a pushing action on the bottom obstacles before swallowing the target and a pushing action on the top one while swallowing the target fruit. 
%The planning strategy although systematic to some extent, it presents some heuristics and defines the pushing action as a vector pointing from the gripper positioning at obstacle level, outside the ROI to the target center. 
In the latter work, the authors adapt a pushing action on the obstacle fruits before swallowing the target. The pushing action results mechanically from the move in a designed direction, thanks to a genuine design of a fingers-like gripper. Although a pushing action is generated along the path to the target, it doesn't rely on the cluster physics, and hence is considered heuristic and limits the picking success rate. In addition, the approach in \cite{xiong2019autonomous} lacks consideration of different kind of occlusions (e.g those coming from stems) which may result in grasp failure due to components coupling, and also, the strategy doesn't consider combined cases (e.g top obstacles on symmetrical side of the target) which can leave the proposed planning strategy without solution.
A recent work, presented in \cite{shyam2019improving}, adopts a probabilistic primitive based optimization technique to generate smooth and fast trajectories for tomato harvesting. Their approach relies on the Covariant Hamiltonian optimization framework for motion planning (\textit{CHOMP}) under obstacle avoidance constraints initialized with a probabilistic primitive. However, it doesn't consider the problem of motion planning for picking in clusters.
%to get closer to the optimal solution with a reduced computation time that basic \textit{CHOMP} takes to converge. 

In parallel to robot harvesting, current works in agrifood-robotics include but are not limited to, weed detection and removal \cite{tellaeche2008vision}, crops growth monitoring through aerial robots (e.g. using quadcopters)\cite{roldan2016heterogeneous}, fruits \cite{kirk2020b} and plants \cite{yamamoto2016node}, \cite{tabb2017robotic} detection and tracking, mobile robot navigation and mapping \cite{nardi2019actively}-\cite{fentanes20183}. Another agri-robotics area is focusing more on robot kinematics and manipulation trying to find a suitable and efficient gripper design 
%\cite{blanes2011technologies}. 
Some grippers are developed to achieve stable and soft contacts \cite{elgeneidy2019characterising} with the fruits and others are developed based on a scissor-like concept \cite{xiong2019development}. 
%In \cite{wang2016design}, the authors developed a clamping mechanism for fruit holding able to separate the fruit from its stem during the picking operation.

%From a perception perspective, Amy Tabb in \cite{tabb2013shape} uses a minimum local search method to reconstruct thin, texture-less objects, like leafless trees, for robotic pruning. In addition, Tabb et al. in \cite{tabb2017robotic} presented a robotic vision system that reconstruct tree traits (e.g branch diameter, length, angle). Michaels et al. in \cite{michaels2015vision} presented a vision-based high speed manipulation system on the mobile robot BoniRob for high precision weed control. Their system relies on a visual servoing technique applied to a delta robot.  

For general applications, many works in motion planning derive from learning techniques. As an example, movement pimitives (MPs) are commonly used for representing and learning basic movements in robotics \cite{paraschos2013probabilistic}. Works as in \cite{paraschos2013probabilistic} and \cite{maeda2017probabilistic} have presented the probabilistic movement primitives framework as a method to encode variability and uncertainty in the movements and to derive new operations which are essential for implementing modulation of a movement, coupling, co-activation, temporal scaling, etc.

Inspired by \cite{shyam2019improving}, in this paper we propose a probabilistic primitive-based planning strategy, however, one that features pushing actions in clusters. We steer the proposed planning strategy towards the current main challenge in fruit harvesting and experiment it in strawberry harvesting. Hence, we present i) typical cluster configurations, ii) a solution to generate pushing actions in a small space region from a number of basis functions, iii) the pushing planner algorithm that generates interactive movement primitives systematically, iv) a simulated field scenario where we tested our approach on three types of clusters. 
% While keeping the optimization of our approach to a future work,   
 %The main problem can be defined by the difficulties to swallow a ripe fruit from its surrounding which can result in a limited harvesting success rate. 
 
% \subsection*{Our approach and contributions}
%Hence, we propose a planning strategy that features a systematic pushing action on the surrounding of a goal ripened fruit. The strategy inherits properties from expert demonstrations and hence generates smooth trajectories that reach the ripened fruit and pick it with a high success rate. 

%\subsection*{Future works}
The rest of the paper is divided into the following: section \ref{sec:prob} defines the problem and the current main challenge in fruit harvesting, section \ref{sec:approach} presents the approach we followed to tackle the problem, section \ref{sec:exp} illustrates experimental results reported on a simulated field and section \ref{sec:conc} concludes with future works.    





